CIM-MLC: A Multi-level Compilation Stack for Computing-In-Memory Accelerators

In recent years, various computing-in-memory (CIM) processors have been presented, showing superior performance over traditional architectures. To unleash the potential of various CIM architectures, such as device precision, crossbar size, and crossbar number, it is necessary to develop compilation tools that are fully aware of the CIM architectural details and implementation diversity. However, due to the lack of architectural support in current popular open-source compiling stacks, existing CIM designs either manually deploy networks or build their own compilers, which is time-consuming and labor-intensive. Although some works expose the specific CIM device programming interfaces to compilers, they are often bound to a fixed CIM architecture, lacking the flexibility to support the CIM architectures with different computing granularity. On the other hand, existing compilation works usually consider the scheduling of limited operation types (such as crossbar-bound matrix-vector multiplication). Unlike conventional processors, CIM accelerators are featured by their diverse architecture, circuit, and device, which cannot be simply abstracted by a single level if we seek to fully explore the advantages brought by CIM. Therefore, we propose CIM-MLC, a universal multi-level compilation framework for general CIM architectures. We first establish a general hardware abstraction for CIM architectures and computing modes to represent various CIM accelerators. Based on the proposed abstraction, CIM-MLC can compile tasks onto a wide range of CIM accelerators having different devices, architectures, and programming interfaces. More importantly, compared with existing compilation work, CIM-MLC can explore the mapping and scheduling strategies across multiple architectural tiers, which form a tractable yet effective design space, to achieve better scheduling and instruction generation results.

==> 3.3.2_optimizationFlow.tex <==
\subsubsection{Multi-level Scheduling Flow}
As shown in \fig\ref{figopt} (d)-(f), our multi-level scheduling scheme will be applied according to the computing abstraction of CIM accelerators. 
When the CIM accelerator only has the CM mode, \name conducts the computation graph (CG-grained) optimization that explores the optimal scheduling policy of the DNN operator on cores and generates the \mp flow. 
If the CIM accelerator has the XBM abstraction, we perform CG-grained optimization and then MVM-grained optimization to fully explore the available resource and computing scheduling as the MVM-grained operation can further explore the high-efficiency scheduling of MVM on crossbars after the scheduling of operators is determined by CG-grained optimization. Then, the resulting \mp flow are generated.
For the CIM accelerator has the WLM mode, we will use the VMM-grained optimization after the CG-grained and MVM-grained optimization has been conducted. Thus, we explore the opportunities of improving computing efficiency by managing rows/buffers in the crossbars. Finally, we obtain the \mp flow as the scheduling results.


With our multi-level scheduling optimization, we can efficiently obtain a scheduling result 
for the CIM with a specific computing granularity that is represented by corresponding computing mode abstraction, avoiding the difficulty that the fine-grained scheduling space is too complex.


==> utility/macro.tex <==
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\etal{\emph{et al}\onedot}
\def\ie{\emph{i.e}\onedot,\xspace} 
\def\Ie{\emph{I.e}\onedot,\xspace}
\def\eg{\emph{e.g}\onedot,\xspace} 
\def\Eg{\emph{E.g}\onedot,\xspace}

\def\etc{\emph{etc}\onedot} 
\def\mp{meta-operator~} 
\def\mps{meta-operators~} 
\def\naive{na\"{\i}ve\xspace}

\def\relu{\textsl{ReLu}} % options: \textit, texttt, \textsf, \textrm, 
\def\pooling{\textsl{pooling}}
\def\softmax{\textsl{Softmax}}

\newcommand{\name}[0]{CIM-MLC~}
\newcommand{\names}[0]{CIM-MLC}
%% comments
\newcommand{\diff}[1]{\textcolor{blue}{#1}}
\newcommand{\addsec}[1]{\textcolor{blue}{#1}}

%% notations
\def\sec{Section~}
\def\secs{Sections~}
\def\eqn{Equation~}
\def\eqns{Equations~}
\def\fig{Figure~}
\def\figs{Figures~}
\def\tab{Table~}
\def\tabs{Tables~}
\def\alg{Algorithm~}
\def\line{Line~}

